Order Optimal Information Spreading Using Algebraic Gossip

In this paper we study gossip based information spreading with bounded message sizes. We use algebraic gossip to disseminate $k$ distinct messages to all $n$ nodes in a network. For arbitrary networks we provide a new upper bound for uniform algebraic gossip of $O((k+\log n + D)\Delta)$ rounds with high probability, where $D$ and $\Delta$ are the diameter and the maximum degree in the network, respectively. For many topologies and selections of $k$ this bound improves previous results, in particular, for graphs with a constant maximum degree it implies that uniform gossip is \emph{order optimal} and the stopping time is $\Theta(k + D)$. To eliminate the factor of $\Delta$ from the upper bound we propose a non-uniform gossip protocol, TAG, which is based on algebraic gossip and an arbitrary spanning tree protocol $\S$. The stopping time of TAG is $O(k+\log n +d(\S)+t(\S))$, where $t(\S)$ is the stopping time of the spanning tree protocol, and $d(\S)$ is the diameter of the spanning tree. We provide two general cases in which this bound leads to an order optimal protocol. The first is for $k=\Omega(n)$, where, using a simple gossip broadcast protocol that creates a spanning tree in at most linear time, we show that TAG finishes after $\Theta(n)$ rounds for any graph. The second uses a sophisticated, recent gossip protocol to build a fast spanning tree on graphs with large weak conductance. In turn, this leads to the optimally of TAG on these graphs for $k=\Omega(\mathrm{polylog}(n))$. The technique used in our proofs relies on queuing theory, which is an interesting approach that can be useful in future gossip analysis.

==> fig/paper_flowchart.tex <==
\scalebox{0.85}{\begin{tikzpicture}

\tikzstyle{block} = [rectangle, draw, fill=blue!20, 
    text width=12em, text centered, rounded corners, minimum height=4em]
    
\def\mydist{4}

\draw[fill=green!15, rounded corners,draw=green!60] (-3,2.2) rectangle (15,-0.4*\mydist);
\node at (6,1.7) (a) {Main Results};

\draw[fill=green!15, rounded corners,draw=green!60] (-3,1.5-\mydist) rectangle (15,-0.4*\mydist-1.7*\mydist);
\node at (6,1-\mydist) (b) {Secondary Results};

\draw[fill=green!15, rounded corners,draw=green!60] (-3,1.5-3.3*\mydist+2.5) rectangle (15,-0.4*\mydist-4.8*\mydist-1);
\node at (0,1-3.3*\mydist+2.5) (c) {Appendix};

\node at (0,0) [block] (1a) {Corollary \ref{col:optimal_algo}: Algebraic gossip with the round-robin gossip broadcast $\mathcal{B_{\mathcal{RR}}}$ and $n$ messages, is $O(n)$};
\node at (6,0) [block] (1) {Theorem \ref{thm:opt_gossip}: Algebraic gossip with some gossip broadcast $\mathcal{B}$ and $k$ messages, is $O(k+\log n +t(\mathcal{B}))$};
\node at (12,0) [block] (2) {Theorem \ref{thm:algebraic_gossip_with_k}: Algebraic gossip with $k$ messages, is $O((k+\log n+D)\Delta)$};

\node at (0,-\mydist) [block] (3) {Theorem \ref{thm:linear_broadcast}: Broadcast with $\mathcal{RR}$ is $O(n)$};
\node at (0,-1.7*\mydist) [block] (4) {Lemma \ref{lemma:sum_of_degrees_on_shortest_path}: Sum of degrees along any shortest path is $\ge 3n$};

\node at (12,-\mydist) [block] (5) {Theorem \ref{thm:tree_of_queues}: Queuing system in a tree topology. All customers leave via the root after $O((k+\log n+l_{max})/\mu)$};

\def\myMoreOffset{1}

\node at (6,-2.5*\mydist-\myMoreOffset) [block] (6) {Corollary \ref{corollary:tree_is_slower_than_line}: Line topology with all customers at the last queue finishes later than the tree topology.};
\node at (12,-2.5*\mydist-\myMoreOffset) [block] (7) {Lemma \ref{lemma:line_stopping_time_with_k}: Using Jackson, line with all customers in the last queue finishes after $O((k+\log n+l_{max})/\mu)$};

\node at (0,-3.5*\mydist-\myMoreOffset) [block] (8) {Lemma \ref{lemma:idle_server}: Tree topology finishes later if the servers do not work all the time.};
\node at (6,-3.5*\mydist-\myMoreOffset) [block] (9) {Lemma \ref{lemma:tree_as_line}: Tree topology with servers that do not work all the time, finishes at the same time as the line.};
\node at (12,-3.5*\mydist-\myMoreOffset) [block] (10) {Lemma \ref{corollary:take_all_customers_back}: Line finishes later if we move all the customers to the last queue.};

\node at (0,-4.2*\mydist-\myMoreOffset) [block] (11) {Lemma \ref{lemma:later_arrivals}: Later arrivals yield later departures};
\node at (12,-4.2*\mydist-\myMoreOffset) [block] (12) {Lemma \ref{lemma:move_one_customer_back}: Line finishes later if we move one customer to the backward queue.};

\node at (0,-4.8*\mydist-\myMoreOffset) [block] (13) {Stochastic dominance definition \ref{dfn:stoch_dom} and claims.};

\path[->] (5) edge (1);
\path[->] (5) edge (2);
\path[->] (4) edge (3);
\path[->] (3) edge (1a);
\path[->] (1) edge (1a);
\path[->] (6) edge (5);
\path[->] (7) edge (5);
\path[->] (8) edge (6);
\path[->] (9) edge (6);
\path[->] (10) edge (6);
\path[->] (11) edge (8);
\path[->] (12) edge (10);
\path[->] (11) edge (12);
\path[->] (13) edge (11);

\end{tikzpicture}}
